Contrastive-mixup learning for improved speaker verification

This paper proposes a novel formulation of prototypical loss with mixup for speaker verification. Mixup is a simple yet efficient data augmentation technique that fabricates a weighted combination of random data point and label pairs for deep neural network training. Mixup has attracted increasing attention due to its ability to improve robustness and generalization of deep neural networks. Although mixup has shown success in diverse domains, most applications have centered around closed-set classification tasks. In this work, we propose contrastive-mixup, a novel augmentation strategy that learns distinguishing representations based on a distance metric. During training, mixup operations generate convex interpolations of both inputs and virtual labels. Moreover, we have reformulated the prototypical loss function such that mixup is enabled on metric learning objectives. To demonstrate its generalization given limited training data, we conduct experiments by varying the number of available utterances from each speaker in the VoxCeleb database. Experimental results show that applying contrastive-mixup outperforms the existing baseline, reducing error rate by 16% relatively, especially when the number of training utterances per speaker is limited.

==> 5_results_main.tex <==
%------------------------------------------------------------------------------------------------------------------------%
\section{Results}
\label{sec:conclusion}
The essence of mixup operation lies in the linear interpolation of sample/label pairs. Thus, it is of key importance that how to generate the interpolation coefficient $\lambda$. As shown in Table 2, when training with the entire VoxCeleb2 dataset, we observe moderate improvement of beta distribution as compared to uniform distribution. Moreover, the smallest VEER, 2.14, is achieved when $\lambda$ is generated using beta(0.1, 0.1), which results in 5.3 \% reduction compared to the basaeline VEER. The authors in \cite{thulasidasan2020mixup} show that relatively smaller values of $\alpha \in [0.1, 0.4]$ gave the best performing results for classification, whereas high values of $\alpha$ resulted in significant under-fitting. In this work, we observed the similar trend where uniform distribution leads to substantial performance degradation.

\begin{table}[!t]
    \small
    \centering
    \caption{Results of beta distribution vs uniform distribution for sampling $\lambda$}
    \addtolength{\tabcolsep}{-2pt}
    \begin{tabular}{lcccc}
    \toprule
    Description & $\lambda$ & \makecell[c]{Loss\\ function} & EER & \makecell[c]{Relative\\ change} \\
    \midrule
    Baseline & - & Original AP & 2.26 & - \\
    \midrule
    \multirow{2}{*}{\makecell[l]{Contrastive mixup}} & Beta(0.1, 0.1) & (\ref{eq:cm_loss}) & 2.14 & - \\
    \cmidrule{4-5}
    & & (\ref{eq:ap_loss}) & 2.09 & - \\
    \bottomrule
    \end{tabular}
    \label{tab:contrastive_up}
\end{table}


% \begin{table}[t]
%     \small
%     \centering
%     \caption{Results of beta distribution vs uniform distribution for sampling $\lambda$}
%     \addtolength{\tabcolsep}{-2pt}
%     \begin{tabular}{lcccc}
%     \toprule
%     Description & $\lambda$ & \makecell[c]{Loss\\ function} & EER & \makecell[c]{Relative\\ change} \\
%     \midrule
%     Baseline & - & Original AP & 2.26 & - \\
%     \midrule
%     \multirow{3}{*}{\makecell[l]{Beta\\distribution}} & Beta(0.1, 0.1) & \multirow{4}{*}{Mixup AP} & 2.14 & +5.3\% \\
%     \cmidrule{2-2} \cmidrule{4-5}
%     & Beta(0.2, 0.2) & & 2.23 & +1.3\% \\
%     \cmidrule{2-2} \cmidrule{4-5}
%     & Beta(0.4, 0.4) & & 2.44 & -8.0\% \\
%     \cmidrule{1-2} \cmidrule{4-5}
%     \makecell[l]{Uniform\\distribution} & Beta(1, 1) & & 3.12 & -86\% \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:tab1}
% \end{table}

To access the performance of contrastive mixup on small datasets, we train quarter ResNet-34 model with limited utterances as shown in Table 3. Here, we find that contrastive mixup can improve speaker verification models by reducing the baseline VEER by up to 12.9\%.  


\begin{table}[t]
    \small
    \centering
    \caption{Comparison of contrastive-mixup loss and original AP loss on small datasets.}
    \addtolength{\tabcolsep}{1pt}
    \begin{tabular}{lccc}
    \toprule
    \makecell[l]{Utterances\\ per speaker} & \makecell[c]{Baseline\\ EER} & \makecell[c]{Mixup\\ EER} & \makecell[c]{Relative\\ change} \\
    \midrule
    2 & 14.57 & 12.69 & +12.9\% \\
    3 & 11.94 & 10.45 & +12.5\% \\
    5 & 9.41 & 8.25 & +12.3\% \\
    10 & 6.69 & 6.06 & +9.4\% \\
    All VoxCeleb2 & 2.26 & 2.09 & +7.5\% \\
    \bottomrule
    \end{tabular}
    \label{tab:tab2}
\end{table}
\rr{Replace change with improvement in the Table~\ref{tab:tab2}?}

In Table~\ref{tab:online_aug}, contrastive mixup is applied on top of online augmentation to further improve the performance of speaker verification systems. In those experiments, we fine tune the mixing coefficient by choosing beta(0.6, 0.6) for 2 utterances, beta(0.2, 0.2) for 3 utterances, beta(0.4, 0.4) for 5 utterances, and beta(0.1, 0.1) for 10 utterances. While contrastive mixup is better compared to the baseline, adding contrastive mixup on top of online augmentation results in additional improvement on all limited cases. 


\begin{table}[t]
    \small
    \centering
    \caption{Comparison of mixup on top of online augmentation}
    \addtolength{\tabcolsep}{-2pt}
    \begin{tabular}{lcccc}
    \toprule
    \makecell[l]{Utterances\\ per speaker} & \makecell[c]{Baseline\\ EER} & \makecell[c]{Mixup\\ EER} & \makecell[c]{Augmentation\\ EER} & \makecell[c]{Mixup + Augmentation \\ EER} \\
    \midrule
    2 & 14.57 & 12.69 & 11.54 & 10.80 \\
    3 & 11.94 & 10.45 & 9.76 & 9.52 \\
    5 & 9.41 & 8.25 & 7.76 & 7.66 \\
    10 & 6.69 & 6.06 & 5.83 & 5.61 \\
    \bottomrule
    \end{tabular}
    \label{tab:online_aug}
\end{table}


